Scatter Correction in X-ray CT by Physics-Inspired Deep Learning

Scatter due to interaction of photons with the imaged object is a fundamental problem in X-ray Computed Tomography (CT). It manifests as various artifacts in the reconstruction, making its abatement or correction critical for image quality. Despite success in specific settings, hardware-based methods require modification in the hardware, or increase in the scan time or dose. This accounts for the great interest in software-based methods, including Monte-Carlo based scatter estimation, analytical-numerical, and kernel-based methods, with data-driven learning-based approaches demonstrated recently. In this work, two novel physics-inspired deep-learning-based methods, PhILSCAT and OV-PhILSCAT, are proposed. The methods estimate and correct for the scatter in the acquired projection measurements. Different from previous works, they incorporate both an initial reconstruction of the object of interest and the scatter-corrupted measurements related to it, and use a deep neural network architecture and cost function, both specifically tailored to the problem. Numerical experiments with data generated by Monte-Carlo simulations of the imaging of phantoms reveal consistent improvement over a recent purely projection-domain deep neural network scatter correction method.

==> paper_old.tex <==
% \documentclass[journal,twoside,web]{ieeecolor}
% \pdfoutput=1
% \usepackage{generic}
% \usepackage{cite}
% \usepackage{amsmath,amssymb,amsfonts}
% \usepackage{standalone}
% \usepackage{algorithm}
% \usepackage{graphicx}
% \usepackage{textcomp}
% \usepackage{algpseudocode}

% % \usepackage{subfigure}
% \usepackage{subcaption,tikz,lipsum}
% \usepackage{lscape}  % Useful for wide tables or figures.
% \usepackage{booktabs}
% \usepackage[utf8]{inputenc}
% \usepackage{longtable}
% \setlength{\marginparwidth}{1.2cm}
% \usepackage[textsize=scriptsize,textwidth=1.4cm]{todonotes}
% \usepackage{makecell}%To keep spacing of text in tables
% % \usepackage[export]{adjustbox}
% % \usepackage[export]{adjustbox}
% \usepackage{wrapfig}


% \def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
%     T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
% % Alter some LaTeX defaults for better treatment of figures:
%     % See p.105 of "TeX Unbound" for suggested values.
%     % See pp. 199-200 of Lamport's "LaTeX" book for details.
%     %   General parameters, for ALL pages:
%     \renewcommand{\topfraction}{0.9}	% max fraction of floats at top
%     \renewcommand{\bottomfraction}{0.8}	% max fraction of floats at bottom
%     %   Parameters for TEXT pages (not float pages):
%     \setcounter{topnumber}{2}
%     \setcounter{bottomnumber}{2}
%     \setcounter{totalnumber}{4}     % 2 may work better
%     \setcounter{dbltopnumber}{2}    % for 2-column pages
%     \renewcommand{\dbltopfraction}{0.9}	% fit big float above 2-col. text
%     \renewcommand{\textfraction}{0.07}	% allow minimal text w. figs
%     %   Parameters for FLOAT pages (not text pages):
%     \renewcommand{\floatpagefraction}{0.7}	% require fuller float pages
% 	% N.B.: floatpagefraction MUST be less than topfraction !!
%     \renewcommand{\dblfloatpagefraction}{0.7}	% require fuller float pages

% 	% remember to use [htp] or [htpb] for placement
	
% \usepackage{scalerel,stackengine}
% \stackMath
% \newcommand\reallywidehat[1]{%
% \savestack{\tmpbox}{\stretchto{%
%   \scaleto{%
%     \scalerel*[\widthof{\ensuremath{#1}}]{\kern.1pt\mathchar"0362\kern.1pt}%
%     {\rule{0ex}{\textheight}}%WIDTH-LIMITED CIRCUMFLEX
%   }{\textheight}% 
% }{2.4ex}}%
% \stackon[-6.9pt]{#1}{\tmpbox}%
% }


% \newcommand{\defsign}{\triangleq}
% \newcommand{\Radon}{\mathcal{R}}
% \newcommand{\FBP}{\reallywidehat{\Radon^{-1}}}


% \markboth{Iskender and Bresler
% :  Scatter Correction in X-Ray CT by Physics-Inspired Deep Learning}
% {Iskender and Bresler
% :  Scatter Correction in X-Ray CT by Physics-Inspired Deep Learning}
% \begin{document}

% \title{Scatter Correction in X-Ray CT \\by Physics-Inspired Deep Learning}
% \author{
% Berk Iskender and Yoram Bresler
% \thanks{This work was supported in part by the NSF under Grant IIS 14-47879, and by US Army MURI Award W911NF-15-1-0479.
%  } 
% \thanks{Berk Iskender and Yoram Bresler are with the Department of Electrical and Computer Engineering, and the Coordinated Science Laboratory, University of Illinois at Urbana-Champaign, Urbana, IL 61801 USA. 
% (e-mail: berki2@illinois.edu; ybresler@illinois.edu)}
%  \vspace*{-1cm}}

% \maketitle
% %\vspace*{-2cm}

% \input{abstract}

% \begin{IEEEkeywords}
% Computed tomography, neural network, CNN, Monte-Carlo, parallel beam, cone beam.
% \end{IEEEkeywords}

% \input{intro}

% \input{background}

% \input{proposed_algorithms}

% \input{methodology}

% \input{experiments}

% \input{conclusions}
% % \medskip

% \bibliographystyle{IEEEtran}
% \small{\bibliography{refs}}

% \input{appendix}

% \end{document}
